Causal inference with recurrent and competing events

Many research questions concern treatment effects on outcomes that can recur several times in the same individual. For example, medical researchers are interested in treatment effects on hospitalizations in heart failure patients and sports injuries in athletes. Competing events, such as death, complicate causal inference in studies of recurrent events because once a competing event occurs, an individual cannot have more recurrent events. Several statistical estimands have been studied in recurrent event settings, with and without competing events. However, the causal interpretations of these estimands, and the conditions that are required to identify these estimands from observed data, have yet to be formalized. Here we use a formal framework for causal inference to formulate several causal estimands in recurrent event settings, with and without competing events. We clarify when commonly used classical statistical estimands can be interpreted as causal quantities from the causal mediation literature, such as (controlled) direct effects and total effects. Furthermore, we show that recent results on interventionist mediation estimands allow us to define new causal estimands with recurrent and competing events that may be of particular clinical relevance in many subject matter settings. We use causal directed acyclic graphs and single world intervention graphs to illustrate how to reason about identification conditions for the various causal estimands based on subject matter knowledge. Furthermore, using results on counting processes, we show that our causal estimands and their identification conditions, which are articulated in discrete time, converge to classical continuous time counterparts in the limit of fine discretizations of time.

==> pgflibraryshapes.swigs.code.tex <==
%%%%
%%% swig  shapes
%%% code for creating multi-part nodes corresponding to split ellipses with a gap
%%%
%%% swig hsplit  : ellipse split horizontally
%%% swig vsplit  : ellipse split vertically
%%%
%%%
%%% Modified from the file: 
%%% pgflibraryshapes.multipart.code.tex (Copyright 2007 by Till Tantau and Mark Wibrow)
%%% 
%%% Copyright 2018 Thomas S. Richardson

% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% swig horizontal split
%%% This is a multi-part node consisting of an ellipse split horizontally into 
%%% upper and lower parts

%%Very useful code allows groups of options to be set as: [...  shape=swig hsplit, swig hsplit={ .... }]
\pgfkeys{/tikz/swig hsplit/.code={%
              \pgfkeys{/tikz/swig hsplit/.cd,#1}%  
               }}%
%\pgfkeys{/tikz/swig hsplit/color/.initial = black}%
\pgfkeys{/tikz/swig hsplit/line color upper/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig hsplit/line color lower/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig hsplit/fill color upper/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig hsplit/fill color lower/.initial = \pgfutil@empty}%
%\pgfkeys{/tikz/swig hsplit/gap/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig hsplit/gap/.initial = 1.0em}
\pgfkeys{/tikz/swig hsplit/line width upper/.initial = \the\pgflinewidth}%
\pgfkeys{/tikz/swig hsplit/line width lower/.initial = \the\pgflinewidth}%
\pgfkeys{/tikz/swig hsplit/inner line width upper/.initial = 0pt}%
\pgfkeys{/tikz/swig hsplit/inner line width lower/.initial = 0pt}%
%\pgfkeys{/pgf/ellipse splitb/dash/.initial = {{{0.5cm}{0.5cm}{0.1cm}{0.2cm}}{0cm}}

\newbox\pgfnodepartlowerbox  %%Associated with anchor "upper"; see pgfmanual3.1, page 1035
\newbox\pgfnodepartupperbox  %%Associated with anchor "lower"; see pgfmanual3.1, page 1035
%%% Every node must have a center anchor
%%% See pgf manual 3.1; p.1036

\pgfdeclareshape{swig hsplit}{%
	\nodeparts{upper,lower}%
	\savedanchor\upper{%
	\pgf@x0pt\pgf@y0pt\relax%
	}%
%https://tex.stackexchange.com/questions/21555/using-patterns-inside-pgf-shapes
	\savedmacro\uppercolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig hsplit/line color upper}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@strokecolor\pgfutil@empty%if not defined even with draw=
	                  \def\uppercolor{.}%
	                \else%
	                    \def\uppercolor{\tikz@strokecolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\uppercolor{\expandafter\pgfkeysvalueof{/tikz/swig hsplit/line color upper}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
	  \savedmacro\lowercolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig hsplit/line color lower}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@strokecolor\pgfutil@empty%if not defined even with draw=
	                  \def\lowercolor{.}%
	                \else%
	                    \def\lowercolor{\tikz@strokecolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\lowercolor{\expandafter\pgfkeysvalueof{/tikz/swig hsplit/line color lower}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
%	
\savedmacro\upperfillcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig hsplit/fill color upper}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@fillcolor\pgfutil@empty%if not defined even with fill=
	                  \def\upperfillcolor{white}%
	                \else%
	                    \def\upperfillcolor{\tikz@fillcolor}% if defined with fill=
	                \fi%
	              \else%
	               \def\upperfillcolor{\expandafter\pgfkeysvalueof{/tikz/swig hsplit/fill color upper}}%if defined
	              \fi}%
\savedmacro\lowerfillcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig hsplit/fill color lower}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@fillcolor\pgfutil@empty%if not defined even with fill=
	                  \def\lowerfillcolor{white}%
	                \else%
	                    \def\lowerfillcolor{\tikz@fillcolor}% if defined with fill=
	                \fi%
	              \else%
	               \def\lowerfillcolor{\expandafter\pgfkeysvalueof{/tikz/swig hsplit/fill color lower}}%if defined
	              \fi}%
	%
        \savedanchor\linewidthupper{%
       \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%
       \pgfmathsetlength\pgf@x{0pt}%
        }%
         \savedanchor\linewidthlower{%
       \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%
       \pgfmathsetlength\pgf@x{0pt}%
        }%
	\savedanchor\gap{% This is a coordinate, but \pgf@x is redundant
	                   \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig hsplit/gap}}%
%%%%%%%% 
	\pgfmathsetlength\pgf@x{0pt}%
	}
	\savedanchor\radii{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y2.0\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%Added to allow for different widths
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%% of lines upper and lower
		\ifdim\pgf@yb>\pgf@ya%
			\pgf@ya\pgf@yb%
		\fi%
		\advance\pgf@y.5\pgf@ya% 
		\pgf@xa.5\wd\pgfnodepartupperbox%
		\pgf@xb.5\wd\pgfnodepartlowerbox%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@xb\pgf@x%
		\pgf@ya\ht\pgfnodepartupperbox%
		\advance\pgf@ya\dp\pgfnodepartupperbox%
		\pgf@yb\ht\pgfnodepartlowerbox%
		\advance\pgf@yb\dp\pgfnodepartlowerbox%
		\advance\pgf@ya\pgf@y%
		\advance\pgf@yb\pgf@y%
		\ifdim\pgf@xa>\pgf@xb%
			\pgf@x1.414213\pgf@xa%
		\else%
			\pgf@x1.414213\pgf@xb%
		\fi%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y1.414213\pgf@ya%
		\else%
			\pgf@y1.414213\pgf@yb%
		\fi%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%
		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
	}
	\savedanchor\lower{%
		\pgf@x-.5\wd\pgfnodepartlowerbox%
		\advance\pgf@x.5\wd\pgfnodepartupperbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y-2.0\pgf@y%
		%\advance\pgf@y-\pgflinewidth%
		\advance\pgf@y-\dp\pgfnodepartupperbox%
		\advance\pgf@y-\ht\pgfnodepartlowerbox%
		%%%%%%
	                   \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/gap}}%
		 %%%%%%%
		\advance\pgf@y-\pgf@ya%	%% Added by TSR for gap
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
	}
	\savedanchor\uppercenterpoint{% NOTE: *Not* the same as anchor "upper center" (this saved anchor is in the middle of the line)
		\pgf@x.5\wd\pgfnodepartupperbox%
		\pgfmathsetlength\pgf@y{-\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y-\dp\pgfnodepartupperbox%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%%%
		\advance\pgf@y-.5\pgf@ya%
	}%
\savedanchor{\greaterlinewidth}{%since seemingly hard to include conditional calculations in anchors (!)
	\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%
	\pgfmathsetlength{\pgf@x}{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%% 
	\ifdim\pgf@xa>\pgf@x%
         \pgf@x\pgf@xa%
         \fi%
         \pgf@y0pt%
}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodepartupperbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\gapcenter{%
	\pgf@x.5\wd\pgfnodepartupperbox%
	\pgfmathsetlength\pgf@y{-\pgfkeysvalueof{/pgf/inner ysep}}%
	\advance\pgf@y-\dp\pgfnodepartupperbox%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%%%
	\advance\pgf@y-.75\pgf@ya%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%%%
	\advance\pgf@y.25\pgf@ya%
	%%%%%%%
	                   \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/gap}}%
	%%%%%%%
	\advance\pgf@y-.5\pgf@ya%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%Added to allow for different widths
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%% of lines upper and lower
	}%
	\savedanchor\basepointlower{%
		\pgf@x.5\wd\pgfnodepartupperbox%
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y-2.0\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
		\advance\pgf@y-\dp\pgfnodepartupperbox%
		\advance\pgf@y-\ht\pgfnodepartlowerbox%
		%%%%%%%%%
	                   \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/gap}}%
		%%%%%%%%%%
		\advance\pgf@y-\pgf@ya%	%% Added by TSR for gap
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodepartupperbox%
		\pgfmathsetlength\pgf@y{.5ex}%
	}%
	\savedanchor\midpointlower{%
		\pgf@x.5\wd\pgfnodepartupperbox% Note: Origin is SW corner of upper text box
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y-2.0\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}%%% 
		\advance\pgf@y-0.5\pgf@ya%
		\advance\pgf@y-\dp\pgfnodepartupperbox%
		\advance\pgf@y-\ht\pgfnodepartlowerbox%
		%%%%%%%%%
	                   \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig hsplit/gap}}%
		%%%%%%%%%%
		\advance\pgf@y-\pgf@ya%	
		\pgfmathsetlength\pgf@ya{.5ex}%
		\advance\pgf@y\pgf@ya%
	}%
	\anchor{upper center}{\linewidthupper\pgf@ya-.5\pgf@y\uppercenterpoint\advance\pgf@y\pgf@ya}
	%%% Required see PGF Manual p.1036
	\anchor{center}{\gapcenter}
	\anchor{lower center}{\linewidthlower\pgf@ya.5\pgf@y\gap\advance\pgf@ya-\pgf@y\uppercenterpoint\advance\pgf@y\pgf@ya}%
	%\pgfpointadd{\uppercenterpoint}{\gap\pgf@y-\pgf@y}}
	\anchor{lower}{\lower}
	\anchor{upper}{\upper}
	\anchor{text}{\upper}
	\anchor{lower base}{\basepointlower}
	\anchor{lower mid}{\midpointlower}
	\anchor{mid}{\midpoint}
	\anchor{mid east}{\greaterlinewidth\pgf@xa.5\pgf@x\radii\advance\pgf@xa\pgf@x\midpoint\advance\pgf@x\pgf@xa}
	\anchor{mid west}{\greaterlinewidth\pgf@xa.5\pgf@x\radii\advance\pgf@xa\pgf@x\midpoint\advance\pgf@x-\pgf@xa}
	\anchor{upper base}{\basepoint}
	\anchor{base}{\basepoint}
	\anchor{base east}{\greaterlinewidth\pgf@xa.5\pgf@x\radii%call \radii;  this sets pgf@x and pgf@y
				\advance\pgf@xa\pgf@x%store pgf@x into pgf@xa
				\basepoint %call \basepoint; this sets pgf@x and pgf@y
	\advance\pgf@x\pgf@xa}  %  Add \pgf@xa to contents of \pgf@x (!!)
%%															
	\anchor{base west}{\greaterlinewidth\pgf@xa.5\pgf@x\radii\advance\pgf@xa\pgf@x\basepoint\advance\pgf@x-\pgf@xa}
	\anchor{north}{\linewidthupper\pgf@ya.5\pgf@y\radii\advance\pgf@ya\pgf@y\uppercenterpoint\advance\pgf@y\pgf@ya}%
	%\pgfpointadd{\uppercenterpoint}{\radii\pgf@x0pt}}%
	\anchor{south}{\linewidthlower\pgf@ya-.5\pgf@y\gap\advance\pgf@ya-\pgf@y\radii\advance\pgf@ya-\pgf@y\uppercenterpoint\advance\pgf@y\pgf@ya}%
	%\pgfpointadd{\uppercenterpoint}{\radii\pgf@ya-\pgf@y\gap\pgf@y-\pgf@y\advance\pgf@y\pgf@ya\pgf@x0pt}}%
	\anchor{west}{\pgfpointadd{\gapcenter}{\greaterlinewidth%
									\pgf@xa-.5\pgf@x%
									\radii%
									\pgf@x-\pgf@x%
									\advance\pgf@x\pgf@xa%
									\pgf@y0pt}}%
	\anchor{east}{\pgfpointadd{\gapcenter}{\greaterlinewidth%
									\pgf@xa.5\pgf@x%
									\radii%
									\advance\pgf@x\pgf@xa%
									\pgf@y0pt}}%
	\anchor{upper east}{\pgfpointadd{\uppercenterpoint}{\linewidthupper\pgf@xa\pgf@y\radii\pgf@y0pt\advance\pgf@x.5\pgf@xa}}%%% %
	\anchor{upper west}{\pgfpointadd{\uppercenterpoint}{\linewidthupper\pgf@xa\pgf@y\radii\pgf@x-\pgf@x\pgf@y0pt\advance\pgf@x-0.5\pgf@xa}}%	
	\anchor{lower west}{\pgfpointadd{\uppercenterpoint}{\linewidthlower\pgf@xa\pgf@y\radii\pgf@xb-\pgf@x\advance\pgf@xb-0.5\pgf@xa\gap\pgf@y-\pgf@y\pgf@x\pgf@xb}}%
	\anchor{lower east}{\pgfpointadd{\uppercenterpoint}{\linewidthlower\pgf@xa\pgf@y\radii\pgf@xb\pgf@x\advance\pgf@xb0.5\pgf@xa\gap\pgf@y-\pgf@y\pgf@x\pgf@xb}}%
	\anchor{north west}{\pgfpointadd{\uppercenterpoint}{\linewidthupper\pgf@ya\pgf@y%
	                                 \radii\advance\pgf@x.5\pgf@ya\advance\pgf@y.5\pgf@ya%
	                                 \pgf@x-0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south west}{\pgfpointadd{\uppercenterpoint}{\linewidthlower\pgf@ya\pgf@y%
					\radii\advance\pgf@x.5\pgf@ya\advance\pgf@y.5\pgf@ya%
					\pgf@xa-0.707106\pgf@x\pgf@ya-0.707106\pgf@y%
					\gap\pgf@y-\pgf@y\advance\pgf@y\pgf@ya\pgf@x\pgf@xa}}%
	\anchor{north east}{\pgfpointadd{\uppercenterpoint}{\linewidthupper\pgf@ya\pgf@y%
					\radii\advance\pgf@x.5\pgf@ya\advance\pgf@y.5\pgf@ya%
                                   	\pgf@x0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south east}{\pgfpointadd{\uppercenterpoint}{\linewidthlower\pgf@ya\pgf@y%
					\radii\advance\pgf@x.5\pgf@ya\advance\pgf@y.5\pgf@ya%
					\pgf@xa0.707106\pgf@x\pgf@ya-0.707106\pgf@y%
					\gap\pgf@y-\pgf@y\advance\pgf@y\pgf@ya\pgf@x\pgf@xa}}%
%%%%%%%%% START OF DRAWING HSPLIT
%%%% Upper
\beforebackgroundpath{%
        \edef\defaultpgflinewidth{\the\pgflinewidth}% store default line width
	 \pgfsetstrokecolor{\uppercolor}%
	  \pgfsetfillcolor{\upperfillcolor}%
	         \expandafter\pgfsetlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig hsplit/line width upper}}%
	          \expandafter\pgfsetinnerlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig hsplit/inner line width upper}}%
		\radii%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgfpathmoveto{\uppercenterpoint\advance\pgf@x-\pgfutil@tempdima}%
		\pgfpatharcaxes{180}{0}{\pgfpoint{\the\pgfutil@tempdima}{0pt}}{\pgfpoint{0pt}{\the\pgfutil@tempdimb}}%
		\pgfpathclose
		\pgfusepath{stroke,fill}
%%%%%% Lower
  \pgfsetlinewidth\defaultpgflinewidth% Reset \the\pgflinewidth to default value (in case changed while drawing upper)
   % \expandafter\pgfsetstrokecolor\expandafter{\pgfkeysvalueof{/tikz/swig hsplit/line color lower}}% old approach
  \pgfsetstrokecolor{\lowercolor}%
    \pgfsetfillcolor{\lowerfillcolor}%
                  \expandafter\pgfsetlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig hsplit/line width lower}}% original
                    \expandafter\pgfsetinnerlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig hsplit/inner line width lower}}%
               	\radii%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgfpathmoveto{\uppercenterpoint\pgf@xa\pgf@x\pgf@ya\pgf@y\advance\pgf@xa\pgfutil@tempdima%
		\gap\advance\pgf@ya-\pgf@y%
		\pgf@x\pgf@xa\pgf@y\pgf@ya%
		}%
		\pgfpatharcaxes{180}{360}{\pgfpoint{-\the\pgfutil@tempdima}{0pt}}{\pgfpoint{0pt}{\the\pgfutil@tempdimb}}%
		\pgfpathclose%
		\pgfusepath{stroke,fill}%
	}
	\anchorborder{%
  	\pgfextract@process\externalpoint{}%  %https://tex.stackexchange.com/questions/255492/storing-a-pgfpoint-for-repeated-use
	%%%%%   This stores the current \pgf@x and \pgf@y in the macro \externalpoint
	\linewidthupper%
	\pgf@ya\pgf@y%
  		\radii%
	\advance\pgf@x.5\pgf@ya% add half-line width to x radius
	\advance\pgf@y.5\pgf@ya% add line width to y radius
  	\edef\pgf@marshal{%
   		\noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
   			{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\uppercenterpoint}%
   	}%  
   	\pgf@marshal%
	\pgf@xa\pgf@x% store the border point
	\pgf@ya\pgf@y% store the border point
	\uppercenterpoint%
	\pgf@yb\pgf@y% store center for upper ellipse
	\pgf@xb\pgf@x% store center for upper ellipse
	\ifdim\pgf@ya<\pgf@yb% if the borderpoint is below center of upper ellipse
% if the border point is below bottom of upper ellipse start over 
%	                                         %the lower ellipse start over (since lower ellipse may have different thickness)
		\linewidthlower%
			\pgf@ya\pgf@y%
  			\radii%
			\advance\pgf@x.5\pgf@ya% add half-line width to x radius
			\advance\pgf@y.5\pgf@ya% add half line width to y radius
  			\edef\pgf@marshal{%
   			\noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
   			{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\uppercenterpoint}%
   			}%  
   			\pgf@marshal%
			\pgf@xa\pgf@x% store the border point
			\pgf@ya\pgf@y% store the border point
			\gap%
			\advance\pgf@ya-\pgf@y%  move y coord of border point down
	\fi%
	\pgf@x\pgf@xa% 
	\pgf@y\pgf@ya% 
  }%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% swig vertical split
%%% This is a multi-part node consisting of an ellipse split vertically into 
%%% left and right parts
%%% The text boxes adjust to the size of the text contained in them
%%% (The split may be off-center in order to keep the ellipse smaller.)


%%%%% START OF V-SPLIT SWIG
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%Very useful code allows groups of options to be set as: [...  shape=swig vsplit, swig vsplit={ .... }]
\pgfkeys{/tikz/swig vsplit/.code={%
              \pgfkeys{/tikz/swig vsplit/.cd,#1}%  
               }}%
\pgfkeys{/tikz/swig vsplit/line color left/.initial = \pgfutil@empty}%    
\pgfkeys{/tikz/swig vsplit/line color right/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig vsplit/fill color left/.initial = \pgfutil@empty}%    
\pgfkeys{/tikz/swig vsplit/fill color right/.initial = \pgfutil@empty}%
\pgfkeys{/tikz/swig vsplit/gap/.initial = 0.8em}%
\pgfkeys{/tikz/swig vsplit/line width left/.initial = \the\pgflinewidth}%
\pgfkeys{/tikz/swig vsplit/line width right/.initial = \the\pgflinewidth}%
\pgfkeys{/tikz/swig vsplit/inner line width left/.initial = 0pt}%
\pgfkeys{/tikz/swig vsplit/inner line width right/.initial = 0pt}%
%\pgfkeys{/tikz/swig vsplit/prop/.initial = 0.5}%  

\newbox\pgfnodepartleftbox  %%Associated with anchor "left"; see pgfmanual3.1, page 1035
\newbox\pgfnodepartrightbox %%Associated with anchor "right"; see pgfmanual3.1, page 1035


%%%
%%%
%% Rectangle "box" contents (with gap=0)
%% 0.5 inner xsep + lefttextbox + inner xsep + 0.5 linewidthleft + gap + 0.5 linewidthright + righttextbox + 0.5 innerxsep
%% origin is at left side of lefttextbox
%%%
\pgfdeclareshape{swig vsplit}{%
	\nodeparts{left,right}
	\savedmacro\leftcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig vsplit/line color left}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@strokecolor\pgfutil@empty%if not defined even with draw=
	                  \def\leftcolor{.}%
	                \else%
	                    \def\leftcolor{\tikz@strokecolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\leftcolor{\expandafter\pgfkeysvalueof{/tikz/swig vsplit/line color left}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
	  \savedmacro\rightcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig vsplit/line color right}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@strokecolor\pgfutil@empty%if not defined even with draw=
	                  \def\rightcolor{.}%
	                \else%
	                    \def\rightcolor{\tikz@strokecolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\rightcolor{\expandafter\pgfkeysvalueof{/tikz/swig vsplit/line color right}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
%	
\savedmacro\leftfillcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig vsplit/fill color left}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@fillcolor\pgfutil@empty%if not defined even with draw=
	                  \def\leftfillcolor{white}%
	                \else%
	                    \def\leftfillcolor{\tikz@fillcolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\leftfillcolor{\expandafter\pgfkeysvalueof{/tikz/swig vsplit/fill color left}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
	  \savedmacro\rightfillcolor{%
	       \edef\tikz@temp{\pgfkeysvalueof{/tikz/swig vsplit/fill color right}}%
	          \ifx\tikz@temp\pgfutil@empty\relax% 
	                  \ifx\tikz@fillcolor\pgfutil@empty%if not defined even with draw=
	                  \def\rightfillcolor{white}%
	                \else%
	                    \def\rightfillcolor{\tikz@fillcolor}% if defined with draw=
	                \fi%
	              \else%
	               \def\rightfillcolor{\expandafter\pgfkeysvalueof{/tikz/swig vsplit/fill color right}}%if defined
	              \fi} %%%Important: adding { } around the last def statement would break this
%	
\savedanchor\gap{% This is a coordinate, but \pgf@y is redundant
	\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/swig vsplit/gap}}%
	\pgfmathsetlength\pgf@y{0pt}%
	}%
\savedanchor\linewidthleft{% This is a coordinate, but \pgf@x is redundant
       \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%
       \pgfmathsetlength\pgf@x{0pt}%
        }%
\savedanchor\linewidthright{% This is a coordinate, but \pgf@x is redundant
       \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%
       \pgfmathsetlength\pgf@x{0pt}%
        }%
\savedmacro\vsplitangle{%
		\pgf@xa\wd\pgfnodepartleftbox%
		\pgf@xb\wd\pgfnodepartrightbox%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa1.5\pgf@x% inner xsep only added left of gap
		\advance\pgf@xb1.5\pgf@x% inner xsep only added right of gap
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%Added to allow for different widths
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% of lines upper and lower
		\advance\pgf@xa.5\pgf@ya% Add width of line for left part (strictly, 2x half for each side of left half)
		\advance\pgf@xb.5\pgf@yb% Add width of line for left part (strictly 2x half for each side of right half)
	\pgfmathsetmacro{\vsplitangle}{acos((\pgf@xa-\pgf@xb)/(1.414213*(\pgf@xa+\pgf@xb)))}%
	%\pgfmathsetlength\pgf@x{0pt}%
	%\pgfmathsetlength\pgf@y{0pt}%
	}%
\savedanchor\radii{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		%\pgf@x2.0\pgf@x% outer x sep added to both halves
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%Added to allow for different widths
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% of lines left and right
		\pgf@xa\wd\pgfnodepartleftbox%
		\pgf@xb\wd\pgfnodepartrightbox%
		\advance\pgf@xa1.5\pgf@x% add inner x sep to left half;
		\advance\pgf@xa.5\pgf@ya% Add half width of line for left part 
		\advance\pgf@xb1.5\pgf@x% add inner x sep to right half
		\advance\pgf@xb.5\pgf@yb% Add half width of line for right part 
		\advance\pgf@xb\pgf@xa% add left and right box lengths together
		\pgf@xa.5\pgf@xb% divide by 2
		\pgf@x1.414213\pgf@xa% compute radius (based on intersect of rectangle box and ellipse at 45 degrees
		%%%%%%%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
%%%%
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb\dp\pgfnodepartrightbox%
		\advance\pgf@ya\pgf@y%
		\advance\pgf@yb\pgf@y%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y1.414213\pgf@ya% compute 2x radius
		\else%
			\pgf@y1.414213\pgf@yb% compute 2x radius
		\fi%
		\pgf@y.5\pgf@y % divide by 2
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%
		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
	}%
\savedanchor\left{%
	\pgf@x0pt\pgf@y0pt\relax%
	}%
\savedanchor\right{%
%		%%%%\pgf@x.5\wd\pgfnodepartrightbox%
		\pgf@x\wd\pgfnodepartleftbox%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x2.0\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/gap}}%%% Added by TSR store gap distance in ya register
		\advance\pgf@x\pgf@xa%	%% Added by TSR for gap
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.5\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%%% 
		\advance\pgf@x.5\pgf@xa%
		\pgf@y0pt\relax%
	}%
\savedanchor\centerleftgapside{%
		\pgf@x\wd\pgfnodepartleftbox%
		%\advance\pgf@x\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.5\pgf@xa%
		%%%%% Repeated code fragment to compute max box height
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%
		%%%%% End repeated code fragment to compute box height
	}%
\savedanchor\globalcenterpoint{%
		\pgf@x\wd\pgfnodepartleftbox%
		\pgf@x.5\pgf@x%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x1\pgf@xa% (0.5 x 3)-1 inner xsep since on each side of gap) 
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/gap}}%
		\advance\pgf@x.5\pgf@xa%
		%\advance\pgf@x\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.25\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% 
		\advance\pgf@x.25\pgf@xa%
		\pgf@xa\wd\pgfnodepartrightbox%
		\advance\pgf@x.5\pgf@xa%
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%
	}%
\savedanchor\linewidthatwidestcenter{% coordinate, but x is redundant
% Slightly obsessive check to find either left or right line width
%   Depending on whether left or right contains the vertical radius.                                  
		\pgf@x\wd\pgfnodepartleftbox%
		\pgf@x.5\pgf@x%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x\pgf@xa% (0.5 x 3) -1 inner xsep since on each side of gap) 
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.25\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% of lines left and right
		\advance\pgf@x.25\pgf@xa%
		\pgf@xa\wd\pgfnodepartrightbox%
		\advance\pgf@x.5\pgf@xa% This contains x-coord of left center but this may not be the widest point 
		                                          % if the global center is right of the gap
		\pgf@xa\wd\pgfnodepartleftbox%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa\pgf@xb%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@xa.5\pgf@xb%
		\ifdim\pgf@x>\pgf@xa%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%
		\else
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%
		\fi%
		%
		\pgf@x0pt% 
	}%
\savedanchor\leftcenter{%
		\pgf@x\wd\pgfnodepartleftbox%
		\pgf@x.5\pgf@x%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x\pgf@xa% (0.5 x 3)-0.5 inner xsep since on each side of gap) 
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.25\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% of lines left and right
		\advance\pgf@x.25\pgf@xa%
		\pgf@xa\wd\pgfnodepartrightbox%
		\advance\pgf@x.5\pgf@xa% 
		%% 
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%
	}%
\savedanchor\rightcenter{%
		\pgf@x\wd\pgfnodepartleftbox%
		\pgf@x.5\pgf@x%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x\pgf@xa% (0.5 x twice inner xsep since on each side of gap) 
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/gap}}% for right center
		\advance\pgf@x\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x.25\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%% of lines left and right
		\advance\pgf@x.25\pgf@xa%
		\pgf@xa\wd\pgfnodepartrightbox%
		\advance\pgf@x.5\pgf@xa% 
		%% 
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%
	}%	
\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodepartleftbox%
		\pgf@y0pt\relax%
	}%
\savedanchor\basepointright{%
		\pgf@x\wd\pgfnodepartleftbox%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x2.0\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/gap}}%%% Added by TSR store gap distance in ya register
		\advance\pgf@x\pgf@xa%	%% Added by TSR for gap
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x0.5\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%%% 
		\advance\pgf@x0.5\pgf@xa%	
		\advance\pgf@x.5\wd\pgfnodepartrightbox%
		\pgf@y0pt\relax%	
	}%
\savedanchor\midpointleft{%
		\pgf@x.5\wd\pgfnodepartleftbox%
		%%%% Repeated code fragment for max box height
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%
	}%
\savedanchor\midpointright{%
			\pgf@x\wd\pgfnodepartleftbox%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x2.0\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/gap}}%%% Added by TSR store gap distance in ya register
		\advance\pgf@x\pgf@xa%	%% Added by TSR for gap
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%%% 
		\advance\pgf@x0.5\pgf@xa%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%%% 
		\advance\pgf@x0.5\pgf@xa%	
		\advance\pgf@x.5\wd\pgfnodepartrightbox%
		%%%% Repeated code fragment for max box height
		\pgf@ya\ht\pgfnodepartleftbox%
		\advance\pgf@ya-\dp\pgfnodepartleftbox%
		\pgf@yb\ht\pgfnodepartrightbox%
		\advance\pgf@yb-\dp\pgfnodepartrightbox%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y.5\pgf@ya% 
		\else%
			\pgf@y.5\pgf@yb% 
		\fi%	
	}%
%%%%%%%%%%%  ANCHORS	
	%% Note: anchors left center and right center are the center of the left and right sides of the gap
	%% These are not the same as saved anchors leftcenter and right center which are the centers of the left and right ellipse
	\anchor{left center}{\linewidthleft\pgf@xa.5\pgf@y\centerleftgapside\advance\pgf@x\pgf@xa}
	\anchor{right center}{\linewidthright\pgf@xa-.5\pgf@y\gap\advance\pgf@xa\pgf@x\centerleftgapside\advance\pgf@x\pgf@xa}
	\anchor{left ellipse center}{\leftcenter}
	\anchor{right ellipse center}{\rightcenter}
	\anchor{left north}{\radii%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgf@ya*(sin(\vsplitangle))}%
		\linewidthleft\advance\pgf@ya.5\pgf@y%
		\centerleftgapside\advance\pgf@y\pgf@ya%
		}%
	\anchor{left south}{\radii%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgf@ya*(sin(\vsplitangle))}%
		\linewidthleft\advance\pgf@ya.5\pgf@y%
		\centerleftgapside\advance\pgf@y-\pgf@ya%
		}%
	\anchor{right north}{\pgfpointadd{\centerleftgapside}{%
	        \radii%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgf@ya*(sin(\vsplitangle))}%
		\linewidthright\advance\pgf@ya.5\pgf@y%
		\gap\pgf@y\pgf@ya%
		}}%
	\anchor{right south}{\pgfpointadd{\centerleftgapside}{%
	        \radii%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgf@ya*(sin(\vsplitangle))}%
		\linewidthright\advance\pgf@ya.5\pgf@y%
		\gap\pgf@y-\pgf@ya%
		}}%
	\anchor{left}{\left}
	\anchor{text}{\left} %Added for compatibility (?)
	\anchor{right}{\right}
	\anchor{center}{\globalcenterpoint}
	\anchor{right base}{\basepointright}
	\anchor{left base}{\basepoint}
	\anchor{base}{\basepoint} %% Added for compatibility
	\anchor{right mid}{\midpointright}
	\anchor{left mid}{\midpointleft}
	\anchor{mid}{\midpointleft}
	\anchor{mid east}{\pgfpointadd{\rightcenter}{\radii\pgf@xa\pgf@x\linewidthright\pgf@x.5\pgf@y\advance\pgf@xa\pgf@x\midpointright\pgf@x\pgf@xa}}%
	\anchor{mid west}{\pgfpointadd{\leftcenter}{\radii\pgf@xa\pgf@x\linewidthleft\pgf@x.5\pgf@y\advance\pgf@xa\pgf@x\midpointleft\pgf@x-\pgf@xa}}%
	\anchor{base east}{\pgfpointadd{\rightcenter\pgf@y0pt}{\radii\pgf@xa\pgf@x\linewidthright\pgf@x.5\pgf@y\advance\pgf@x\pgf@xa\pgf@y0pt}}%
	\anchor{base west}{\pgfpointadd{\leftcenter\pgf@y0pt}{\radii\pgf@xa\pgf@x\linewidthleft\pgf@x.5\pgf@y\advance\pgf@xa\pgf@x\pgf@x-\pgf@xa\pgf@y0pt}}%
		%\anchor{mid west}{\radii\pgf@xa\pgf@x\centerleftgapside\advance\pgf@x-\pgf@xa}
	\anchor{base}{\basepoint}
	\anchor{north}{\pgfpointadd{\globalcenterpoint}{\linewidthatwidestcenter\pgf@ya\pgf@y\radii\advance\pgf@y.5\pgf@ya\pgf@x0.0pt}}%
	\anchor{south}{\pgfpointadd{\globalcenterpoint}{\linewidthatwidestcenter\pgf@ya\pgf@y\radii\pgf@y-\pgf@y\advance\pgf@y-.5\pgf@ya\pgf@x0pt}}% 
	\anchor{east}{\pgfpointadd{\rightcenter}{\radii\pgf@xa\pgf@x\linewidthright\pgf@x.5\pgf@y\advance\pgf@x\pgf@xa\pgf@y0pt}}%
	\anchor{west}{\pgfpointadd{\leftcenter}{\radii\pgf@xa-\pgf@x\linewidthleft\pgf@x-.5\pgf@y\advance\pgf@x\pgf@xa\pgf@y0pt}}%	
	\anchor{north west}{\pgfpointadd{\leftcenter}{\linewidthleft\pgf@xa.5\pgf@y%
	          \radii\advance\pgf@x\pgf@xa\advance\pgf@y\pgf@xa%
	          \pgf@x-0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south west}{\pgfpointadd{\leftcenter}{\linewidthleft\pgf@xa.5\pgf@y%
	          \radii\advance\pgf@x\pgf@xa\advance\pgf@y\pgf@xa%
	          \pgf@x-0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
	\anchor{north east}{\pgfpointadd{\rightcenter}{\linewidthright\pgf@xa.5\pgf@y%
	          \radii\advance\pgf@x\pgf@xa\advance\pgf@y\pgf@xa%
	          \pgf@x0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south east}{\pgfpointadd{\rightcenter}{\linewidthright\pgf@xa.5\pgf@y%
	          \radii\advance\pgf@x\pgf@xa\advance\pgf@y\pgf@xa%
	          \pgf@x0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
%%%%%%%%% START OF DRAWING VSPLIT
%%%%% Left
\beforebackgroundpath{%
         \edef\defaultpgflinewidth{\the\pgflinewidth}% store default line width
          \pgfsetstrokecolor{\leftcolor}%
           \pgfsetfillcolor{\leftfillcolor}%
	 % \expandafter\pgfsetstrokecolor\expandafter{\pgfkeysvalueof{/tikz/swig vsplit/linecolorleft}}%
	         \expandafter\pgfsetlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig vsplit/line width left}}%
	               \expandafter\pgfsetinnerlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig vsplit/inner line width left}}%
		\radii%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@ya{\pgf@ya*(sin(\vsplitangle))}%% compute y distance for off-center split
		\pgfpathmoveto{\centerleftgapside\advance\pgf@y\pgf@ya}% set path to centerpoint + \pgf@ya
		\pgfpatharcaxes{\vsplitangle}{360-\vsplitangle}{\pgfpoint{\the\pgfutil@tempdima}{0pt}}{\pgfpoint{0pt}{\the\pgfutil@tempdimb}}%
		\pgfpathclose
		\pgfusepath{stroke,fill}
%%%%%% right
     \pgfsetlinewidth\defaultpgflinewidth % Reset \the\pgflinewidth to default value (in case changed while drawing left)
                 \pgfsetstrokecolor{\rightcolor}%
                 \pgfsetfillcolor{\rightfillcolor}%
                    \expandafter\pgfsetlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig vsplit/line width right}}%
                    \expandafter\pgfsetinnerlinewidth\expandafter{\pgfkeysvalueof{/tikz/swig vsplit/inner line width right}}%
		\radii%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgf@ya\pgf@y%
		\pgfmathsetlength\pgf@yb{\pgf@ya*(sin(\vsplitangle))}%% compute y distance for off-center split
		\pgfpathmoveto{\centerleftgapside\pgf@xa\pgf@x\pgf@ya\pgf@y\advance\pgf@ya\pgf@yb%
		\gap\advance\pgf@xa\pgf@x%
		\pgf@x\pgf@xa\pgf@y\pgf@ya%
		}%
		\pgfpatharcaxes{\vsplitangle}{-\vsplitangle}{\pgfpoint{\the\pgfutil@tempdima}{0pt}}{\pgfpoint{0pt}{\the\pgfutil@tempdimb}}%
		\pgfpathclose%
		\pgfusepath{stroke,fill}%
	}
	\anchorborder{%
  	\pgfextract@process\externalpoint{}%  %https://tex.stackexchange.com/questions/255492/storing-a-pgfpoint-for-repeated-use
	%%%%%   This stores the current \pgf@x and \pgf@y in the macro \externalpoint
	\linewidthleft%
	\pgf@ya\pgf@y%
  		\radii%
	\advance\pgf@x.5\pgf@ya% add half-line width to x radius
	\advance\pgf@y.5\pgf@ya% add half line width to y radius
  	\edef\pgf@marshal{%
   		\noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
   			{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\leftcenter}%
   	}%  
   	\pgf@marshal%
	\pgf@xa\pgf@x% store the border point
	\pgf@ya\pgf@y% store the border point
	\centerleftgapside%
	\pgf@xb\pgf@x% point on gap
	\ifdim\pgf@xa>\pgf@xb%
		\linewidthright%
		\pgf@ya\pgf@y%
  		\radii%
		\advance\pgf@x.5\pgf@ya% add half-line width to x radius
		\advance\pgf@y.5\pgf@ya% add half line width to y radius
  		\edef\pgf@marshal{%
   			\noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
   				{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\rightcenter}%
   	}%  
	\pgf@marshal%
	\else
	\pgf@x\pgf@xa% 
	\pgf@y\pgf@ya% 
	\fi%
  }%
}


\endinput

